D2P-Fed: Differentially Private Federated Learning With Efficient Communication

In this paper, we propose the discrete Gaussian based differentially private federated learning (D2P-Fed), a unified scheme to achieve both differential privacy (DP) and communication efficiency in federated learning (FL). In particular, compared with the only prior work taking care of both aspects, D2P-Fed provides stronger privacy guarantee, better composability and smaller communication cost. The key idea is to apply the discrete Gaussian noise to the private data transmission. We provide complete analysis of the privacy guarantee, communication cost and convergence rate of D2P-Fed. We evaluated D2P-Fed on INFIMNIST and CIFAR10. The results show that D2P-Fed outperforms the-state-of-the-art by 4.7% to 13.0% in terms of model accuracy while saving one third of the communication cost.

==> binom_thm.tex <==
\section{Communication Cost \& MSE of Binomial Mechanism}

For completeness, we also include the communication cost and MSE of Binomial mechanism under stochastic uniform quantization and random rotation.
%
We denote Binomial mechanism with stochastic uniform quantization with $\pi_{k,q, binom}$ and random rotation with $\pi_{k,q, binom}^{(rot)}$. 

% \begin{theorem}[Communication cost of $\pi_{k,q, binom}$]
% If $X^{\max}=D$, then the mean estimate is unbiased and
% \begin{equation*}
%     \mathcal{E}(\pi_{k,q, binom}, X_1^n)\leq \frac{dD^2}{n(k-1)^2} + \frac{d}{n}\cdot \frac{4mp(1-p)D^2}{(k-1)^2}
% \end{equation*}
% \end{theorem}

\begin{theorem}[MSE of $\pi_{k,q, binom}$]
If $X^{\max}=D$, then the mean estimate is unbiased and
\begin{equation*}
    \mathcal{E}(\pi_{k,q, binom}, X_1^n)\leq \frac{dD^2}{n(k-1)^2} + \frac{d}{n}\cdot \frac{4mp(1-p)D^2}{(k-1)^2}
\end{equation*}
\end{theorem}

% \begin{theorem}[Communication cost of $\pi_{k,q, binom}^{(rot)}$]
% If $X^{\max}=D$, then the mean estimate is unbiased and
% \begin{equation*}
%     \mathcal{E}(\pi_{k,q, binom}, X_1^n)\leq \frac{dD^2}{n(k-1)^2} + \frac{d}{n}\cdot \frac{4mp(1-p)D^2}{(k-1)^2}
% \end{equation*}
% \end{theorem}

\begin{theorem}[MSE of $\pi_{k,q, binom}^{(rot)}$]
For any $\delta$, let $X^{\max}=2D\sqrt{\frac{\log(2nd/\delta)}{d}}$, then 
\begin{equation*}
    \mathcal{E}(\pi_{k,q, binom}^{(rot)}, X_1^n)\leq \frac{2\log\frac{2nd}{\delta}}{n(k-1)^2} + \frac{8\log\frac{2nd}{\delta}\cdot mp(1-p)D^2}{n(k-1)^2}+4D^2\delta^2
\end{equation*}
and the bias is $\leq 2D\delta$.
\end{theorem}


==> comm.tex <==
\section{Communication Protocol}

We inherit the stochastic rotated quantization protocol from \cite{mcmahan2016communication} in our protocol.
%
We first briefly review the communication protocol including vanilla stochastic uniform quantization and random rotation.
%
After that, we augment the protocol with the discrete Gaussian mechanism and the secure aggregation and analyze the mean square error (MSE) of our protocol.
%
We also provide per-round communication cost and mean squared error analysis for both our protocol and \cite{agarwal2018cpsgd}.
%
At last, we relates the convergence rate of the learning protocol with the mean squared error using Theorem~\ref{thm:converge} (\cite{agarwal2018cpsgd}) and analyze the total communication cost under the same mean squared error.
%
The result shows that because discrete Gaussian mechanism supports tighter composition than Binomial mechanism, the noise added is smaller, the convergence is faster and the total communication cost is better.

\subsection{Notation}

Before we dive into the details of the communication protocol, we first introduce the notations we use.
%
Let $\pi$ denote the communication protocol and each client holds a vector $X_i$.
%
The communication cost for each client is $\mathcal{C}(\pi, X_i)$ and the total communication cost $\mathcal{C}(\pi, X_1^n)=\sum_{i=1}^n\mathcal{C}(\pi, X_i)$.
%
Let $\bar{X}$ denote the actual mean value of these vectors $\bar{X}=\frac{1}{n}\sum_{i=1}^nX_i$ and $\hat{\bar{X}}$ denote the output of the protocol.
%
The mean squared error between the estimation and the actual mean is represented by $\mathcal{E}(\pi, X_1^n)=\mathbb{E}[\|\hat{\bar{X}}-\bar{X}\|^2]$.
%
We use $X^{\max}$ ($X_i^{\max}$) to denote the upper (lower) bound of the maximum (minimum) value within a vector $X_i$.
%
% Because the gradient is mapped to the quotient group $\mathcal{Z}_{2^q}$

\subsection{Communication Protocol}

\paragraph{Stochastic $k$-level quantization.}
%
Stochastic $k$-level quantization is one of the most widely used quantization scheme.
%
For a $d$-dimensional vector $X$ whose maximum is $X^{\text{max}}=\max_{1\leq j \leq d}X[j]$ and whose minimum is $X^{\text{min}}=\max_{1\leq j \leq d}X[j]$, let $B[r] := X^{\text{min}} + \frac{r(X^{\text{max}}-X^{\text{min}})}{k-1}$ for every $r\in[0,k)$.
%
The scheme quantizes each coordinate $X[j]\in[B[r], B[r+1])$ using the following formula.

\begin{equation*}
Y[j]=\left\{
\begin{aligned}
&B[r] &~~~&\text{w.p.}~\frac{X[j]-B[r]}{B[r+1]-B[r]} \\
&B[r+1] &~~~&\text{o.w.}
\end{aligned}
\right.
\end{equation*}
%
We use $\pi_k$ to denote vanilla stochastic k-level quantization.
As a reult,  we have that $\mathcal{C}(\pi_k, X_1^n)=n\cdot(d\rceil\log_2 k\lceil+\tilde{\mathcal{O}}(1))$ and $\mathcal{E}(\pi_k, X_1^n)=\mathcal{O}(\frac{d}{n}\cdot\frac{1}{n}\sum_{i=1}^n\|X_i\|_2^2)$.
%
However, this vanilla version leaks the exact value of the maximum and minimum within a vector so it is not compatible with output perturbation. 
%
Thus, we use the modified version where $X^{\max}$ is fixed by the server before the protocol and $X^{\max}=-X^{\min}$.

\paragraph{Random Rotation.}
%
Random rotation is a technique initially proposed by \cite{mcmahan2016communication} to reduce the MSE of the stochastic uniform quantization.
%
The key intuition is that the MSE of stochastic uniform quantization is $\mathcal{O}(\frac{d}{n}(X^{\max})^2)$.
With random rotation, we can limit $X^{\max}$ to $\sqrt{\frac{\log d}{d}}$ w.h.p. so the MSE will be improved to $\mathcal{O}(\frac{\log d}{n})$.
%
\cite{agarwal2018cpsgd} also leverages random rotation to reduce MSE.
%
However, in their setting, random rotation intrinsically harms their privacy guarantee because the $l_\infty$-sensitivity might increase with rotation.
%
A natural advantage of discrete Gaussian is that the privacy guarantee only depends on $l_2$-sensitivity which is an invariant under rotation.
%
Thus, random rotation does not harm our privacy guarantee at all.
%
We omit the details here and refer the interested readers to \cite{mcmahan2016communication}.
%
We denote the protocol with $\pi_k^{(rot)}$.
%
We know that $\mathcal{C}(\pi_k^{(rot)}, X_1^n)$ is the same with stochastic random rotation and $\mathcal{E}(\pi_k^{(rot)}, X_1^n)=\mathcal{O}(\frac{\log d}{n}\cdot\frac{1}{n}\sum_{i=1}^n\|X_i\|_2^2)$.

\subsection{Secure Aggregation}
\ruoxi{it will be good if we can briefly give a background on secure aggregation, e.g., its key idea and typical protocol. the ICLR community may not be familiar with it.}

Secure aggregation is another challenge when applying discrete Gaussian in federated learning setting.
%
Because discrete Gaussian contains infinite possible values, it is impossible to encode the noise within finite coding length.
%
One candidate solution is to use variable length encoding (\cite{mcmahan2016communication}).
%
However, it is unclear how to reconcile secure aggregation (\cite{bonawitz2017practical}) with variable length encoding schemes.
%
To address the challenge, we propose to project the involved values into the quotient group.
%
According to the post-processing theorem of RDP (\cite{mironov2017renyi}), the result should still follow rigorous R\'enyi differential privacy.

% \begin{algorithm}%[H]
% \DontPrintSemicolon
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \SetKwProg{Fn}{Function}{:}{\KwRet}
% \SetAlgoLined
% \KwIn{$\mathbb{L}$, $\sigma$, $\mathbb{L}_{q}$: quotient group of $\mathbb{L}$, $\phi$: mapping from $\mathbb{L}$ to $\mathbb{L}_{q}$}
% \For{each client $i\in [m]$}{
%     \For{each client $j\in [m]$ and $j \neq i$}{
%         $\mu_{ij}\sim Unif(\mathbb{L}_{q})$\;
%         Send $\mu_{ij}$ to j\;
%     }
% }
% \For{each client $i\in [m]$}{
%     $\nu_i\sim N_{\mathbb{L}}(\sigma)$\;
%     $\hat{g}_i = \phi(g_i + \nu_i + \sum_{j\neq i}\mu_{ij}-\sum_{j\neq i}\mu_{ji})$\;
%     Send $\hat{g}_i$ to the server\;
% }
% Server computes $\sum_{i\in[m]}\hat{g}_i$\;
% \caption{Distributed mean estimation with discrete Gaussian and secure aggregation.}
% \label{alg:sec_agg}
% \end{algorithm}

\begin{theorem}[RDP for Algorithm~\ref{alg:protocol}]
Algorithm~\ref{alg:protocol} obeys the same RDP guarantee as vanilla global discrete Gaussian mechanism with the same parameters.
\end{theorem}

\begin{proof}[Proof Sketch]
According to modular arithmetic, 
\begin{equation*}
\begin{split}
    \sum_{i\in[m]}\hat{g}_i &= \phi(\sum_{i\in[m]}\phi(\mathcal{R}\times(\psi_k(g_i) + \nu_i) + \sum_{j\neq i}\mu_{ij}-\sum_{j\neq i}\mu_{ji}))\\
    &= \phi(\sum_{i\in[m]}(\mathcal{R}\times(\psi_k(g_i) + \nu_i) + \sum_{j\neq i}\mu_{ij}-\sum_{j\neq i}\mu_{ji}))\\
    &= \phi(\sum_{i\in[m]}(\mathcal{R}\times(\psi_k(g_i) + \nu_i))) = \phi(\mathcal{R}\times\sum_{i\in[m]}(\psi_k(g_i) + \nu_i))
\end{split}.
\end{equation*}
% According to post-processing theorem, the result is ()-RDP.
\end{proof}

Algorithm~\ref{alg:protocol} is a simplified version of the full secure aggregation protocol (\cite{bonawitz2017practical}) and we only use it to clarify the idea behind the reconciliation.
%
Indeed, discrete Gaussian can be used with the complete version of secure aggregation using the same trick.

\subsection{Communication Protocol with Discrete Gaussian Mechanism}

\begin{algorithm}%[H]
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Fn}{Function}{:}{\KwRet}
\SetAlgoLined
\KwIn{$\mathbb{L}=\frac{X^{\max}}{k-1}\mathbb{Z}$, $\sigma$, $\mathbb{L}_{q}=(\mathbb{L}+\frac{q}{2})\mod q$: translated quotient group of $\mathbb{L}$, $\phi$: mapping from $\mathbb{L}$ to $\mathbb{L}_{q}$, $\psi_k$: quantization function, $\mathcal{R}$: rotation matrix}
\For{each client $i\in [m]$}{
    \For{each client $j\in [m]$ and $j \neq i$}{
        $\mu_{ij}\sim Unif(\mathbb{L}_{q})$\;
        Send $\mu_{ij}$ to j\;
    }
}
\For{each client $i\in [m]$}{
    $\nu_i\sim N_{\mathbb{L}}(\sigma)$\;
    $\hat{g}_i = \phi(\mathcal{R}\times(\psi_k(g_i) + \nu_i) + \sum_{j\neq i}\mu_{ij}-\sum_{j\neq i}\mu_{ji})$\;
    Send $\hat{g}_i$ to the server\;
}
Server computes $\sum_{i\in[m]}\hat{g}_i$\;
\caption{The complete distributed mean estimation protocol.}
\label{alg:protocol}
\end{algorithm}

Once we take discrete Gaussian into consideration, secure aggregation technique is a natural requirement to ensure that the server can only view the average gradient.
%
\cite{agarwal2018cpsgd} has the same requirement but they did not discuss the issue explicitly.
%
As pointed out in \cite{bonawitz2017practical}, once combined with secure aggregation, each field has to expand at least $n$ times to prevent overflow of the sum.
%
In this section, we provide per-round communication cost and MSE for both protocols for direct comparison.
%
We denote our protocol as $\pi_{k, q, N_{\mathbb{L}}(\sigma^2)}^{(rot)}$ and the protocol from \cite{agarwal2018cpsgd} as $\pi_{k, Bin(m, p)}^{(rot)}$.

First, we present Theorem 4 from \cite{agarwal2018cpsgd} and correct the per-round communication cost considering secure aggregation.
\begin{theorem}[Modified Theorem 4 from \cite{agarwal2018cpsgd} with secure aggregation]
For any $\delta$, let $X^{\max}=2D\sqrt{\frac{\log(2nd/\delta)}{d}}$, then
\begin{equation*}
    \mathcal{E}(\pi_{k, Bin(m, p)}, X_1^n)\leq \frac{2\log\frac{2nd}{\delta}\cdot D^2}{n(k-1)^2}+\frac{8\log\frac{2nd}{\delta}\cdot mp(1-p)D^2}{n(k-1)^2} + 4D^2\delta^2
\end{equation*}
and the bias is $\leq2D\delta$.
%
Besides,
\begin{equation*}
    \mathcal{C}(\pi_{k,Bin(m,p)}, X_1^n) = n\cdot(d\log(n(k+m)+1) +\tilde{\mathcal{O}}(1)).
\end{equation*}.
\end{theorem}

Next, we present the per-round communication cost and MSE of our protocol.

\begin{theorem}%[Mean squared error]
If we choose $\sigma\geq1\sqrt{2\pi}$, the mean squared error is
\begin{equation*}
    \mathcal{E}(\pi_{k, q}, X_1^n)\leq (1-\frac{1}{1+3e^{-2\pi^2\sigma^2}}(1-\Phi(q)))\cdot\frac{4d(X^{\max})^2}{n(k-1)^2}(\frac{1}{4}+\sigma^2) + (1-\Phi(q-k-1))\cdot q^2
\end{equation*}.
Besides, the per-round communication cost is
\begin{equation*}
    \mathcal{C}(\pi_{k,q}, X_1^n) = n\cdot(d\log( nq+1)+\tilde{\mathcal{O}}(1))
\end{equation*}.
\end{theorem}

\begin{proof}[Proof Sketch]

Before starting the proof, we introduce two lemmas for simplicity of the proof.

\begin{lemma}[Proposition 19 from \cite{canonne2020discrete}]
For all $\sigma\in\mathbb{R}$ with $\sigma>0$,
\begin{equation*}
    \mathbb{V}[N_{\mathbb{Z}}(0,\sigma^2)]\leq\sigma^2(1-\frac{4\pi^2\sigma^2}{e^{4\pi^2\sigma^2-1}})<\sigma^2
\end{equation*}
Moreover, if $\sigma^2\leq \frac{1}{3}$, then $\mathbb{V}[N_{\mathbb{Z}}(0, \sigma^2)]\leq 3\cdot e^{-\frac{1}{2\sigma^2}}$
\label{lem:var}
\end{lemma}

\begin{lemma}[Proposition 23 from \cite{canonne2020discrete}]
For all $m\in\mathbb{Z}$ with $m\geq 1$ and all $\sigma\in\mathbb{R}$ with $\sigma>0$,
\begin{equation*}
    \mathbb{P}_{X\sim N_\mathbb{Z}(0, \sigma^2)}[X\geq m] \leq \mathbb{P}_{X\sim N(0, \sigma^2)}[X\geq m-1].
\end{equation*}
Moreover, if $\sigma\geq 1/\sqrt{2\pi}$, we have 
\begin{equation*}
    \mathbb{P}_{X\sim N_{\mathbb{Z}}(0,\sigma^2)}[X\geq m]\geq \frac{1}{1+3e^{-2\pi^2\sigma^2}}\mathbb{P}_{X\sim N(0,\sigma^2)}[X\geq m]
\end{equation*}
\label{lem:tail_bound}
\end{lemma}

Now we start our proof. 
%
MSE can be rewritten in the following format.
\begin{equation*}
\begin{split}
    \mathbb{E}[\|\hat{\bar{X}}-\bar{X}\|_2^2|]&=\frac{1}{n^2}\sum_{j=1}^d\sum_{i=1}^n\mathbb{E}[(\hat{\bar{X}}_i(j)-X_i(j))^2]\\
\end{split}
\end{equation*}

For each $\star=\mathbb{E}[(\hat{\bar{X}}_i(j)-X_i(j))^2]$
%\ruoxi{$\star = \frac{1}{n^2}\sum_d\sum_n\mathbb{E}[(\hat{\bar{X}}_i(j)-X_i(j))^2]$?}
, we need to consider two cases. 
%
If no overflow happens, due to Lemma~\ref{lem:var}
\begin{equation*}
    \star_{\neg o} 
    \leq \mathbb{E}[(\frac{2X^{\max}}{k-1})^2(\mathbb{V}(Ber(p_i(j)))+\mathbb{V}(N_{\mathbb{L}}(\sigma)))]
    \leq \frac{4(X^{\max})^2}{(k-1)^2}(\frac{1}{4}+\sigma^2)
\end{equation*}
\ruoxi{with random rotation, there is small probability that the l infinity norm bigger than $X^{max}$}
%
If overflow happens, trivially we have $\star_o \leq q^2$. \ruoxi{should the RHS be $k^2$}
Thus, we have
\begin{equation}
    \star = \mathbb{P}[\neg o]\cdot\star_{\neg o} + \mathbb{P}[o]\cdot\star_o \leq \mathbb{P}_{X\sim N_{\mathbb{L}}(\sigma^2)}[X\leq q]\cdot\star_{\neg o} + \mathbb{P}_{X\sim N_{\mathbb{L}}(\sigma^2)}[X\geq q-k]\cdot\star_o
\end{equation}
%
\ruoxi{$P[\neg o] = P[X+N_\mathbb{L}\leq q]$?}
With Lemma~\ref{lem:tail_bound}, we can bound the probabilities and get the final MSE result in the theorem.

\lun{we need to take the overflow probability of random rotation into account.}
\end{proof}

\begin{theorem}
If we clip the $l_2$ norm of the gradient to D, and take $k=\sqrt{d}+1$, then the $l_2$ sensitivity of $\pi_{k}^{(rot)}$ is $4D$.
\label{thm:sensitivity}
\end{theorem}

\begin{proof}
The $l_2$ sensitivity of the gradient is naturally bounded by $2D$.
%
The rotation does not change the sensitivity.
%
The $k$-level quantization might expand the space a little bit as shown in the following figure.
%
A rough upper bound on the radius of the red circle is $D+\sqrt{d}\frac{D}{k-1}$.
%
When we take $k=\sqrt{d}-1$, it reduces to $2D$.
%
Thus, the upper bound on the sensitivity is $4D$.

\tikzset{StyleOne/.style={samples=200, thick}}
\tikzset{StyleTwo/.style={samples=200, dashed}}

\begin{tikzpicture}
\begin{axis}[
    axis lines = middle,
    xlabel = $x$,
    xmax=2,
    xmin=-2,
    minor x tick num={4},
    ylabel = {$y$},
    ymax=2,
    ymin=-2,
    minor y tick num={4},
    grid=both,
    axis equal=true,
    legend style={
        cells={anchor=west},
        legend pos=north west
    },
]

% \addplot [domain=-4:4, My Style, red] {2*x+1};
% \addlegendentry{$y=2x+1$}

\addplot [domain=-1:1, StyleOne, blue] {sqrt(1-x^2)};
\addplot [domain=-1:1, StyleOne, blue] {-sqrt(1-x^2)};
\addlegendentry{clipped gradient space}

\addplot [domain=-1.16619037897:1.16619037897, StyleTwo, red] {sqrt(1.36-x^2)};
\addplot [domain=-1.16619037897:1.16619037897, StyleTwo, red] {-sqrt(1.36-x^2)};
\addlegendentry{quantized gradient space}

\node[circle,fill,red,inner sep=1pt] at (axis cs:0.2,1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:0.4,1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:0.6,1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:0.8,0.8) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:1,0.6) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:1,0.4) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:1,0.2) {};

\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.2,1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.4,1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.6,1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.8,0.8) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-1,0.6) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-1,0.4) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-1,0.2) {};

\node[circle,fill,red,inner sep=1pt] at (axis cs:0.2,-1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:0.4,-1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:0.6,-1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:0.8,-0.8) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:1,-0.6) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:1,-0.4) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:1,-0.2) {};

\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.2,-1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.4,-1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.6,-1) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-0.8,-0.8) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-1,-0.6) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-1,-0.4) {};
\node[circle,fill,red,inner sep=1pt] at (axis cs:-1,-0.2) {};
\end{axis}
\end{tikzpicture}

\end{proof}


% The probability of exceeding $q$ is upper bounded by $\Phi=$.
% %
% Use tail bound for discrete Gaussian.
% %
% Thus we get the final bound as follow.

% \begin{equation*}
% \begin{split}
%     \mathbb{E}[\|\hat{\bar{X}}-\bar{X}\|_2^2]&\leq \frac{4d(X^{\max})^2}{n(k-1)^2}((1-\Phi)(\frac{1}{4}+\sigma)+\Phi\cdot2^q)
% \end{split}
% \end{equation*}

% First, we ignore the effect of secure aggregation and derive the mean squared error of discrete Gaussian mechanism as follow.


\subsection{Total Communication Cost}

First, we relate the convergence rate with mean squared error using Theorem~\ref{thm:converge}.
%

\begin{theorem}[\cite{ghadimi2013stochastic}]
%
Let $F$ be $L$-smooth and $\forall x, \|\nabla F(x)\|\leq D$. Let $w^0$ satisfy $F(w^0)-F(w^*)\leq D_F$. Let $q$ be a quantization scheme, and $\gamma\overset{\Delta}{=}\min\{L^{-1}, \sqrt{2D_F}(\sigma\sqrt{LT})^{-1}\}$, then after $T$ rounds
$$
\mathbb{E}_{t\sim(Unif(T))}[\|\nabla F(w^t)\|_2^2]\leq \frac{2D_FL}{T} + \frac{2\sqrt{2}\sigma\sqrt{LD_F}}{\sqrt{T}}+DB
$$,
where $\sigma^2=\max_{1\leq t\leq T}2\mathbb{E}[\|g^t(w^t)-\nabla F(w^t)\|_2^2]+2\max_{1\leq t\leq T}\mathbb{E}_q[\|g^t(w^t)-\tilde{g}^t(w^t)\|_2^2]$,
and $B=\max_{1\leq t\leq T}\|g^t(w^t)-\tilde{g}^t(w^t)\|$. The expectation in the above equations is over the randomness in gradients and quantization.
\label{thm:converge}
\end{theorem}

As theorem~\ref{thm:converge} indicates, for a given gradient bound, the smaller the MSE is, the fewer rounds are needed.
%
To directly compare our protocol with \cite{agarwal2018cpsgd}, we conduct asymptotic analysis for the MSE with fixed privacy budget, per-round communication cost and the number of communication rounds.

Since we fix the per-round communication cost, $q\approx8\log(2\delta)/\eps$.
%
Thus, $\star_o=?$ is negligible.
%
If the total number of communication rounds are $T$ and the total privacy budget is $(\epsilon, \delta)$, then each round can share $\mathcal{O}(\epsilon)/\sqrt{T}$ budget.
%
Then we consider the effect of subsampling.
%
In \cite{agarwal2018cpsgd}, the privacy amplification of subsampling is $\mathcal{O}(\gamma)$.
%
In our protocol, due to Theorem~\ref{lem:analytica}, the amplification is qudratic $\mathcal{O}(\gamma^2)$.
%
Thus, the variance of the discrete Gaussian noise is $\mathcal{O}(\gamma^2\sqrt{T}/\epsilon)$ while Binomial noise is $\mathcal{O}(\gamma\sqrt{T}/\epsilon)$.
%
It is obvious that our protocol adds a $\gamma$ factor.
%
In typical scenario, $\gamma$ can be chosen from tens to hundreds and the improvement is pretty significant.




% \paragraph{Remark.} Theorem~\ref{thm:converge} relates the convergence to (1) the worst-case mean square error between the quantized mean and the original mean, (2) sub-sampling bias as pointed out in~\cite{agarwal2018cpsgd}.

\paragraph{Composition.} By Lemma~\ref{lm:rdp_composition}, the composition of $T$ $(\alpha,\epsilon)$-DP mechanisms is $(\alpha,T\epsilon)$-DP. Note that $\epsilon$ is a function of $\alpha$ for $1\leq \alpha\leq \infty$, and this function is completely determined by the privacy mechanism. We use the notation $\epsilon(\alpha)$ to emphasize the dependence of $\epsilon$ on $\alpha$. Leveraging the relationship between RDP and DP parameters described in Lemma~\ref{lm:rdp_dp_conversion}, we know that the composition of $T$ $(\alpha,\epsilon)$-RDP mechanisms is also $(T\epsilon(\alpha)+\frac{\log 1/\delta}{\alpha-1},\delta)$-DP. We can now solve the following optimization problem to get the smallest $\epsilon$ for a given desired $\delta$:
\begin{align}
\label{eqn:rdp_dp_opt}
    \epsilon(\delta) = \min_\alpha T\epsilon(\alpha)+\frac{\log \frac{1}{\delta}}{\alpha-1}
\end{align}
Since $\epsilon(\alpha)$ is nondecreasing in $\alpha$~\citep{van2014renyi}, it follows that the optimization problem in (\ref{eqn:rdp_dp_opt}) is unimodal. Hence, the optimizer can be obtained by taking the derivative of (\ref{eqn:rdp_dp_opt}) and setting it to be zero:
\begin{align}
\label{eqn:optimizer}
    T\epsilon'(\alpha) = \frac{\log \frac{1}{\delta}}{(\alpha-1)^2}
\end{align}

\underline{Example: Continous Gaussian Mechanism.} The RDP of the Gaussian mechanism is $\epsilon(\alpha) = \frac{\alpha}{2\sigma^2}$. Using (\ref{eqn:optimizer}), we can derive the optimizer $\alpha^*$ that minimizes the value of $\epsilon$:
\begin{align}
    \alpha^* = \sqrt{\frac{2\sigma^2\log \frac{1}{\delta}}{T}} + 1
\end{align}
Hence, using the conversion from RDP to DP, we can get that for a given desired $\delta$, the smallest $\epsilon$ for the composition of $T$ Gaussian mechanisms with zero mean and $\sigma^2$ variance is 
\begin{align}
    \epsilon(\delta) = 2\sqrt{\frac{T\log \frac{1}{\delta}}{2\sigma^2}} + \frac{1}{2\sigma^2}
\end{align}

Next, we derive the privacy bound of discrete Gaussian under advanced composition.
%
\begin{lemma}[Advanced Composition]
$\forall \epsilon, \delta, \delta'\geq 0$, the class of $(\epsilon, \delta)$-differentially private mechanisms satisfies $(\epsilon', k\delta+\delta')$-differential privacy under $k$-fold adaptive composition for:
\begin{equation*}
    \epsilon'=\sqrt{2k\ln(1/\delta')}\epsilon + k\epsilon(e^{\epsilon}-1).
\end{equation*}
\label{lem:adv_com}
\end{lemma}
%
By Lemma~\ref{lem:adv_com}, the privacy bound of $T$ discrete Gaussian mechanisms under advanced composition is 
\begin{equation*}
123    
\end{equation*}



==> dis_gaussian.tex <==
\section{Discrete Gaussian Mechanism}

In this section, we introduce discrete Gaussian mechanism and provide the R\'enyi differential privacy analysis.

Discrete Gaussian mechanism works by adding noise drawn from calibrated discrete Gaussian distribution (Definition~\ref{def:dg}).

\begin{definition}[Discrete Gaussian Distribution]
Discrete Gaussian is a probability distribution on a discrete additive subgroup $\mathbb{L}$ parameterized by $\sigma$. For a discrete Gaussian distribution $N_{\mathbb{L}}(\sigma)$ and $x\in\mathbb{L}$, the probability mass on $x$ is proportional to $e^{-\pi x^2/(2\pi\sigma^2)}$.
\label{def:dg}
\end{definition}

Variables following discrete Gaussian mechanism have several useful features in distributed mean estimation.
%
For instance, the sum of two discrete Gaussian variables still follows discrete Gaussian distribution (Lemma~\ref{lem:sum}).
%
The dilation of a discrete Gaussian variable still follows discrete Gaussian distribution (Lemma~\ref{lem:dilation}).
%
The proof is straightforward and we omit it here.

\begin{lemma}[Sum of discrete Gaussian variables]
Let $X\sim N_{\mathbb{L}}(\sigma_x)$ and $Y\sim N_{\mathbb{L}}(\sigma_y)$.
%
If a third variable $Z$ is generated by the sum of $X$ and $Y$: $Z=X+Y$, then $Z\sim N_{\mathbb{L}}(\sqrt{\sigma_x^2 + \sigma_y^2})$.
\label{lem:sum}
\end{lemma}

% \begin{proof}[Proof Sketch]
% If we denote the coefficient before the discrete Gaussian probability mass function as $c_\mathbb{L}(\sigma)$, then we have the following result.
% \begin{equation*}
% \begin{split}
%     \mathbb{P}[Z=z] &= \sum_{x\in \mathbb{L}}\mathbb{P}[X=x]\mathbb{P}[Y=z-x]\\ &= c_\mathbb{L}(\sigma_x)c_\mathbb{L}(\sigma_y)(\sum_{x\in\mathbb{L}}\exp(-\frac{(x-\frac{\sigma_x^2z}{\sigma_x^2+\sigma_y^2})^2}{2(\frac{\sigma_x^2\sigma_y^2}{\sigma_x^2+\sigma_y^2})}))\exp(-\frac{z^2}{2\pi(\sigma_x^2+\sigma_y^2)})
% \end{split}
% \end{equation*}

% Because probability mass function is still proportional to $e^{-z^2/(2\pi(\sigma_x^2+\sigma_y^2))}$, it follows $N_{\mathbb{L}}(\sqrt{\sigma_x^2+\sigma_y^2})$.
% \end{proof}

\begin{lemma}[Dilation of discrete Gaussian variables]
Let $X\sim N_{\mathbb{L}}(\sigma)$.
%
If $Z=X/a$, then $Z\sim N_{\mathbb{L}}(\sigma/a)$.
\label{lem:dilation}
\end{lemma}

\cite{canonne2020discrete} prove concentrated differential privacy for discrete Gaussian mechanism.
%
However, there lacks tight composition theorem like moments accountant for concentrated differential privacy.
%
Thus, we provide R\'enyi differential privacy analysis for discrete Gaussian mechanism and use analytical moments accountant (\cite{wang2018subsampled}) for tight composition.

\begin{theorem}[R\'enyi differential privacy for discrete Gaussian mechanism]
If $f$ has sensitivity $1$, then the discrete Gaussian mechanism: $f(\cdot)+N_{\mathbb{L}}(\sigma)$ satisfies $(\alpha, \alpha/(2\sigma^2))$-RDP. 
\label{thm:gdp}
\end{theorem}

\begin{proof}
\begin{equation*}
\begin{split}
    D_\alpha&(N(0, \sigma^2)\|N(\mu, \sigma^2))\\ &= \frac{1}{\alpha-1}\log\sum_{\mathbb{L}}\frac{1}{\sum_{\mathbb{L}}\exp(-(x-\mu)^2/(2\sigma^2))}\exp(-\alpha x^2/(2\sigma^2)\cdot \exp(-(1-\alpha) (x-\mu)^2/(2\sigma^2))\\
    &= \frac{1}{\alpha-1}\log\frac{1}{\sum_{\mathbb{L}}\exp(-(x-\mu)^2/(2\sigma^2))}\sum_{\mathbb{L}}\exp((-x^2+2(1-\alpha)\mu x-(1-\alpha)\mu^2)/(2\sigma^2))\\
    &=\frac{1}{\alpha-1}\log\{\exp((\alpha^2-\alpha)\mu^2/(2\sigma^2))\}\\
    &=\alpha\mu^2/(2\sigma^2)
\end{split}
\end{equation*}
\end{proof}

\begin{lemma}[Analytical moments accountant for Discrete Gaussian mechanism (\cite{wang2018subsampled})]
Given a dataset of $n$ points drawn from a domain $\mathcal{X}$ and a discrete Gaussian mechanism $\mathcal{M}$ that takes an input from $\mathcal{X}^m$ for $m\leq n$, let $\mathcal{M}\circ\emph{subsample}$ be the composition of subsample and $\mathcal{M}$. For all integers $\alpha>2$, if $\mathcal{M}$ obeys $(\alpha, \epsilon(\alpha))$-RDP, then the subsampled discrete Gaussian mechanism $\mathcal{M}\circ \emph{subsample}$ obeys $(\alpha, \epsilon'(\alpha))$-RDP where,
\begin{equation*}
    \epsilon'(\alpha)\leq \frac{1}{\alpha-1}\log(1+\gamma^2{\alpha\choose 2}\min\{4(e^{\epsilon(2)}-1), 2e^{\epsilon(2)}\} + \sum_{j=3}^{\alpha}2\gamma^j{\alpha \choose j}e^{(j-1)\epsilon(j)}).
\end{equation*}
\label{lem:analytical}
\end{lemma}

% \lun{these theorems are directly taken from Yuxiang's paper. Modify a little bit.}

\begin{lemma}[Adaptive composition of RDP (\cite{mironov2017renyi})]
\label{lm:rdp_composition}
If (randomized) mechanism $\mathcal{M}_1$ obeys $(\alpha, \epsilon_1)$-RDP, and $\mathcal{M}_2$ obeys $(\alpha, \epsilon_2)$-RDP, then their composition obeys $(\alpha, \epsilon_1+\epsilon_2)$-RDP.
\end{lemma}

\begin{lemma}[RDP-DP conversion (\cite{mironov2017renyi})]
\label{lm:rdp_dp_conversion}
If $\mathcal{M}$ obeys $(\alpha, \epsilon)$-RDP, then $\mathcal{M}$ obeys $(\epsilon+\log(1/\delta)/(\alpha-1), \delta)$-DP for all $0<\delta<1$.
\end{lemma}

% \lun{what factors do we save compared with advanced composition?}

% \lun{The rest is old stuff. Compare with DeepAI paper and decide whether to keep or discard.}
% \begin{theorem} (Tail Bound for Discrete Gaussian Distribution~(\cite{lyubashevsky2012lattice})).
% For any $k>0$, 
% \begin{enumerate}
%     \item $\forall k>0, \prob[|x|>k\sigma;x\sample D_{\mathbb{L}, \sigma}]\leq 2e^{-\frac{k^2}{2}}$
%     \item $\forall k>1, \prob[\|x\|>k\sigma\sqrt{m};x\sample D^m_{\mathbb{L}, \sigma}]< k^me^{\frac{m}{2}(1-k^2)}$
% \end{enumerate}
% \label{thm:tail}
% \end{theorem}

% \begin{theorem} (Discrete Gaussian Mechanism).
% Let $f: \mathcal{D}\rightarrow\mathbb{L}$ be an arbitrary function with domain $\mathcal{D}$ and range $\mathbb{L}$, and its $l_2$-sensitivity is $\Delta f=\max_{\text{adjacent }x, y}\|f(x)-f(y)\|_2$. The \emph{Discrete Gaussian Mechanism which adds noise scaled to $D_{\mathbb{L}, c\Delta f/\epsilon}$} to $f$ is $(\epsilon, \delta)$-differentially private, where $c^2\geq2\ln\frac{4}{\delta}$.
% \end{theorem}

% \begin{proof}

% We first prove the one-dimensional case. 
% \begin{equation*}
% \begin{split}
%     |\ln\frac{\exp(-\frac{z^2}{2\sigma^2})}{\exp(-\frac{(z+\Delta f)^2}{2\sigma^2})}|=|\frac{2z\Delta f+\Delta^2f}{2\sigma^2}|.
% \end{split}
% \end{equation*}

% This quantity is bound by $\epsilon$ when $z < \sigma^2\epsilon/\Delta f-\Delta f/2$. We then use Theorem~\ref{thm:tail} to bound $\prob[|z|\geq\sigma^2\epsilon/\Delta f-\Delta f/2]$.

% \begin{equation*}
% \begin{split}
%     \prob[z\geq\sigma^2\epsilon/\Delta f-\Delta f/2] \leq \frac{\delta}{2}
%     \Rightarrow \sigma \geq (\sqrt{2\ln\frac{2}{\delta}}+\sqrt{2\ln\frac{2}{\delta}+2\epsilon})\Delta f/ 2\epsilon \Rightarrow \sigma \geq \sqrt{2\ln\frac{2}{\delta}+2\epsilon}\Delta f/ \epsilon
% \end{split}
% \end{equation*}


% In summary, we have proved that with the specified noise parameters, the probability ratio is bounded $e^\epsilon$ with probability $1-\delta$. Thus, one-dimensional Discrete Gaussian mechanism is $(\epsilon, \delta)$-differentially private. Then we extend the result to higher dimenstions. Let $v=f(x)-f(y)$.

% \begin{equation*}
% \begin{split}
%     |\ln\frac{\exp(-\|z\|^2/2\sigma^2)}{\exp(-\|z+v\|^2/2\sigma^2)}|=|\frac{1}{2\sigma^2}(\|z\|^2-\|z+v\|^2|=*
% \end{split}
% \end{equation*}

% The tricky part is $z$ and $v$ may not align.
% %
% We will use the ``somewhat'' symmetric property of multi-dimentional discrete gaussian.
% %
% We take such a basis of the lattice that the first basis vector aligns with $v$ and then do the Graham Schmidt process to find a set of orthogonal vectors (note that these vectors may not be in the lattice).
% %
% We then decompose $z$ to this set of vectors and let $\lambda_1$ denote the projection of $z$ on the first basis.
% %
% \begin{equation*}
%     * \leq |\frac{1}{2\sigma^2}(2\lambda_1\Delta f+\Delta^2 f)| 
% \end{equation*}
% %
% Then the rest of the argument proceeds as above.

% \end{proof}

==> dis_laplace.tex <==
\section{Discrete Laplace Mechanism}

% \lun{One issue about discrete Laplace mechanism is that the sum of Laplace mechanism is not Laplace. Take a look at Poisson distribution and~\cite{dwork2006our}.}

\begin{definition} (Discrete Laplace Distribution~(\cite{inusah2006discrete})).
Discrete Laplace is a probability distribution on $j\mathbb{Z}$ parameterized by precision $j$ and base $p$. The probability mass on $x$ is $\frac{1-p}{1+p}\cdot p^{|x/j|}$, where $p=e^{-j/\sigma}$.
\end{definition}

% \begin{theorem} (Discrete Laplace Mechanism).
%     Let $f: \mathcal{D}\rightarrow\mathbb{L}^d$ be an arbitrary function with domain $\mathcal{D}$ and range $\mathbb{L}^d$, and its $l_1$-sensitivity is $\Delta f=\max_{\text{adjacent }x, y}\|f(x)-f(y)\|_1$.
% %
% The \emph{Discrete Laplace Mechanism} which adds noise scaled to $Lap(\Delta f/\epsilon)$ to $f$ is $(\epsilon, 0)$-differentially private.
% \end{theorem}

% \begin{proof}

% Let $x$ and $y$ be adjacent input pairs\, and $f: \mathcal{D}\rightarrow\mathbb{R}^d$ be some function with $l_1$-sensitivity $1$. 
% %
% Let $p_x$ denote the probability function of $f(x) + Lap(\Delta f/\epsilon)$ and $p_y$ denote the probability function of $f(y) + Lap(\Delta f/\epsilon)$.

% \begin{equation*}
% \begin{split}
%     \frac{p_x(z)}{p_y(z)}= \prod_{i=1}^{d}\frac{p^{-|z-f_i(x)|/j}}{p^{-|z-f_i(y)|/j}}
%     \leq p^{-\|f(x)-f(y)\|_1/j} = \exp(\epsilon)
% \end{split}
% \end{equation*}

% \end{proof}

\begin{theorem} (Discrete Laplace Mechanism).
    Let $f: \mathcal{D}\rightarrow\mathbb{L}^d$ be an arbitrary function with domain $\mathcal{D}$ and range $\mathbb{L}^d$, and its $l_1$-sensitivity is $\Delta f=\max_{\text{adjacent }x, y}\|f(x)-f(y)\|_1$.
%
The \emph{Discrete Laplace Mechanism} which adds noise scaled to $Lap(\Delta f/\epsilon)$ to $f$ is $(\alpha, \frac{1}{\alpha-1}\log\{\frac{\alpha}{2\alpha-1}\exp(\frac{\alpha-1}{\lambda}) + \frac{\alpha-1}{2\alpha-1}\exp(-\frac{\alpha}{\lambda})\})$-R\'enyi differentially private.
\end{theorem}

% \begin{proof}
% \end{proof}

==> old/abstract.tex <==
\begin{abstract}
Ever since its proposal, differential privacy has become the golden standard for rigorous privacy protection.
%
Output perturbation is the most widely used differentially private mechanism.
%
It works by adding calibrated noise drawn from the real domain to the output.
%
However, the finite computers can only represent real numbers to a given machine precision.
%
To guarantee the strictness of differential privacy under fixed precision, several pioneering works (\cite{dwork2006our,ghosh2012universally,balcer2017differential,agarwal2018cpsgd, canonne2020discrete}) proposed to use noise drawn from discrete for differential privacy.
%
However, discrete differentially private mechanisms are not used in dense tasks such as deep learning because of the lack of tight composition theorem like moments accountant.
%
In this paper, we prove R\'enyi differential privacy for discrete Gaussian mechanism.
%
Thus, we can directly use analytical moments accountant (\cite{wang2018subsampled}) to provide tight composition for distributed mean estimation.
\end{abstract}
